MM-Verify: Enhancing Multimodal Reasoning with Chain-of-Thought Verification

According to the Test-Time Scaling, the integration of External Slow-Thinking with the Verify mechanism has been demonstrated to enhance multi-round reasoning in large language models (LLMs). However, in the multimodal (MM) domain, there is still a lack of a strong MM-Verifier. In this paper, we introduce MM-Verifier and MM-Reasoner to enhance multimodal reasoning through longer inference and more robust verification. First, we propose a two-step MM verification data synthesis method, which combines a simulation-based tree search with verification and uses rejection sampling to generate high-quality Chain-of-Thought (COT) data. This data is then used to fine-tune the verification model, MM-Verifier. Additionally, we present a more efficient method for synthesizing MMCOT data, bridging the gap between text-based and multimodal reasoning. The synthesized data is used to fine-tune MM-Reasoner. Our MM-Verifier outperforms all larger models on the MathCheck, MathVista, and MathVerse benchmarks. Moreover, MM-Reasoner demonstrates strong effectiveness and scalability, with performance improving as data size increases. Finally, our approach achieves strong performance when combining MM-Reasoner and MM-Verifier, reaching an accuracy of 65.3 on MathVista, surpassing GPT-4o (63.8) with 12 rollouts.

==> table/orm_bench.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|ccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Models}} & \textbf{Out Judege} & \textbf{TT} & \textbf{TF} \\
    \midrule
    GPT-4o-mini & 61.4  &     -  & - \\
    Gemini-1.5-Pro & 55.0  &     -  & - \\
    Gemini-1.5-Flash & 50.6  &     -  & - \\
    Claude-3.5-sonnet-20240620 & 53.0  &     -  & - \\
    Claude-3-opus-20240229 & 46.7  &     -  & - \\
    Claude-3-sonnet-20240229 & 51.6  &     -  & - \\
    Claude-3-haiku-20240307 & 41.7  &     -  & - \\
    \midrule
    Qwen2-VL-72B-Instruct & 61.3  &     -  & - \\
    Qwen2-VL-7B-Instruct & 46.4  &     -  & - \\
    InternVL-1.5-Chat & 46.8  &     -  & - \\
    MiniCPM-Llama3-V-2.5 & 45.0  &     -  & - \\
    LLaVA-1.6-Mistral-7B-Instruct & 51.2  &     -  & - \\
    Phi-3-Vision-128k-Instruct & 48.6  &     -  & - \\
    CogVLM2-Llama3-Chat-19B & 46.3  &     -  & - \\
    \midrule
    \textbf{Verifier-S.1} & \textbf{61.3}  & \textbf{65.0}  & \textbf{52.1} \\
    \textbf{Verifier-S.2} & \textbf{61.7}  & \textbf{64.3}  & \textbf{53.4} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:orm_bench}%
\end{table}%


==> table/scale_mm.tex <==

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Method} & \textbf{Data} & \textbf{Voting} & \textbf{Verifier-S.1} & \textbf{Verifier-S.2} \\
    \midrule
    \rowcolor[rgb]{ .851,  .882,  .949} \multicolumn{5}{c}{sample 4} \\
    MM-Reasonser & 6,952 & 59.0  & 59.8  & 60.6 \\
    MM-Reasonser & 18,944 & 59.2  & 60.3  & 61.2 \\
    MM-Reasonser & 32,146 & 59.4  & 60.6  & 61.5 \\
    \midrule
    \rowcolor[rgb]{ .851,  .882,  .949} \multicolumn{5}{c}{sample 8} \\
    \midrule
    MM-Reasonser & 6,952 & 60.8  & 62.5  & 62.8 \\
    MM-Reasonser & 18,944 & 61.2  & 62.6  & 63.0 \\
    MM-Reasonser & 32,146 & 62.2  & 63.8  & 65.3 \\
    \midrule
    \rowcolor[rgb]{ .851,  .882,  .949} \multicolumn{5}{c}{sample 12} \\
    \midrule
    MM-Reasonser & 6,952 & 62.6  & 62.8  & 63.4 \\
    MM-Reasonser & 18,944 & 63.0  & 63.8  & 64.7 \\
    MM-Reasonser & 32,146 & 64.6  & 64.8  & 65.2 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:scale_mm}%
\end{table}%

